Improving block-based compensated wavelet lifting by reconstructing unconnected pixels

This paper presents a new approach for improving the visual quality of the lowpass band of a compensated wavelet transform. A high quality of the lowpass band is very important as it can then be used as a downscaled version of the original signal. To adapt the transform to the signal, compensation methods can be implemented directly into the transform. We propose an improved inversion of the block-based motion compensation by processing unconnected pixels by a reconstruction method. We obtain a better subjective visual quality while furthermore saving up to 2.6% of bits for lossless coding.

==> tab/YUV__1002.1__ClassB-BasketballDrive__fs_Lband.tex <==
\textbf{67.45} & 67.52 & +0.10

==> tab/YUV__1002.1__ClassB-BasketballDrive__fs_complete.tex <==
\textbf{145.99} & 146.06

==> tab/YUV__1002.1__ClassB-BasketballDrive__psnr_Lband.tex <==
\textbf{37.6} & 37.3

==> tab/YUV__1003.1__ClassB-BQTerrace__fs_Lband.tex <==
\textbf{322.43} & 323.32 & +0.27

==> tab/YUV__1003.1__ClassB-BQTerrace__fs_complete.tex <==
\textbf{664.95} & 665.83

==> tab/YUV__1003.1__ClassB-BQTerrace__psnr_Lband.tex <==
37.5 & \textbf{37.6}

==> tab/YUV__1004.1__ClassB-Cactus__fs_Lband.tex <==
\textbf{248.74} & 249.16 & +0.17

==> tab/YUV__1004.1__ClassB-Cactus__fs_complete.tex <==
\textbf{515.66} & 516.08

==> tab/YUV__1004.1__ClassB-Cactus__psnr_Lband.tex <==
\textbf{38.7} & 38.5

==> tab/YUV__1005.1__ClassB-Kimono1__fs_Lband.tex <==
\textbf{94.23} & 94.24 & +0.01

==> tab/YUV__1005.1__ClassB-Kimono1__fs_complete.tex <==
\textbf{201.94} & 201.95

==> tab/YUV__1005.1__ClassB-Kimono1__psnr_Lband.tex <==
\textbf{42.1} & 42.0

==> tab/YUV__1006.1__ClassB-ParkScene__fs_Lband.tex <==
\textbf{115.88} & 115.94 & +0.05

==> tab/YUV__1006.1__ClassB-ParkScene__fs_complete.tex <==
\textbf{231.84} & 231.90

==> tab/YUV__1006.1__ClassB-ParkScene__psnr_Lband.tex <==
\textbf{39.9} & \textbf{39.9}
